NeurDB: An AI-powered Autonomous Data System

In the wake of rapid advancements in artificial intelligence (AI), we stand on the brink of a transformative leap in data systems. The imminent fusion of AI and DB (AIxDB) promises a new generation of data systems, which will relieve the burden on end-users across all industry sectors by featuring AI-enhanced functionalities, such as personalized and automated in-database AI-powered analytics, self-driving capabilities for improved system performance, etc. In this paper, we explore the evolution of data systems with a focus on deepening the fusion of AI and DB. We present NeurDB, an AI-powered autonomous data system designed to fully embrace AI design in each major system component and provide in-database AI-powered analytics. We outline the conceptual and architectural overview of NeurDB, discuss its design choices and key components, and report its current development and future plan.

==> cover_letter.tex <==
\newcommand{\comments}[2]{\begin{tcolorbox}[colback=gray!20, colframe=black, sharp corners, width=\textwidth, boxrule=0.2mm]\noindent\emph{Comment #1}: {#2}\end{tcolorbox}}
\newcommand{\response}[2]{\vspace{0mm}\noindent\textbf{Response #1}: {#2} \vspace{0.5mm}}

\newcommand{\commentsmeta}[1]{\noindent\emph{Comment}: \emph{#1}}

\newcommand{\responsemeta}[1]{\vspace{0mm}\noindent\textbf{Response}: {#1} \vspace{0.5mm}}

\newcommand{\revhighlight}[1]{\emph{\textbf{\uuline{#1}}}}
% \pagestyle{empty}
\thispagestyle{empty}


\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{4mm}

% \begin{multicols}{0}

% \noindent To PC co-chairs, meta reviewer, and reviewers:


\noindent We would like to thank the reviewers for their constructive comments and suggestions.
We have addressed all the comments in the revised paper. 
We highlight the major changes made on the manuscript in
{\color{blue} blue}.
% We have listed the major changes below. 


\vspace{-3mm}
\section*{Summary of Changes}
\vspace{-2mm}
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]

\item We have revised Section~\ref{sec:application} to demonstrate how AI-powered applications in the healthcare and e-commerce domains can be potentially built with the unique functionalities of \dbname.

\item We have addressed all the presentation issues as suggested. 
In particular, we have revised the Abstract and Section~\ref{sec:introduction} to define the AI-powered Autonomous Data System more clearly.
We have added the required citation in Section~\ref{subsec:related_work}.
We have updated Figure~\ref{fig:history} and Figure~\ref{fig:overview} to enhance clarity.

\item We have enhanced Section~\ref{subsec:auto_overview} to clarify our approach to addressing the issue that AI models can become inefficient with dynamic workloads.

\end{itemize}
\vspace{-2mm}



% \section*{Response to Associate Editor}
% % \begin{comment}
% \commentsmeta{
% We have now received constructive reviews for this submission. In the reviews, a common concern on the minor presentation issues has been raised. Moreover, the reviewers recommend either a minor revision or an acceptance. Based on these reviews, I recommend that this paper goes through a minor revision to fully address the reviewers’ comments.  
% }
% % \end{comment}


% \responsemeta{
% We have addressed all the minor presentation issues as suggested.
% Furthermore, we have enhanced the paper layout and thoroughly proofread the revised paper.
% For detailed information, please kindly refer to our responses to R1, R2, and R3 below.
% }

\vspace{-3mm}
\section{Response to Reviewer \#1}


\comments{1}{
It is better to provide some potential applications of NeurDB, based on its unique functions.
}


\response{1}{
Following your suggestion, we have improved Section~\ref{sec:application} to outline the AI-powered applications in healthcare and e-commerce domains, and envision how they can be built with the unique functionalities of \dbname.
In addition to providing a mature infrastructure for fast data access and processing, \dbname offers in-database AI-powered analytics, which facilitates the development of complex AI applications and enhances their performance.
}

% In the finance sector, with \dbname, the 
% Predict the income of all male users aged between 20 and 30.
% Healthcare Finance
% Multi-agent
% RAG
% AIGC data - data generator



\comments{2}{
It is better to conduct some experiments to show the performance of NeurDB.
}

\response{2}{
We would like to clarify that this paper is not a full paper. It primarily focuses on positioning \dbname, our next-generation data system designed to fully embrace AI in each major system component and provide in-database AI-powered analytics.
As mentioned in Section~\ref{sec:overview}, realizing \dbname requires significant effort in developing various techniques and evaluating \dbname necessitates a comprehensive approach that considers efficiency, security, scalability, etc. 
To maintain a clear focus on system positioning, we chose not to include experiments in this paper.
However, we would like to note that some key techniques used in \dbname have already been published and evaluated.
For example, in the paper published in VLDB'24 [5], we have tested the model selection technique presented in Section~\ref{subsec:selection}.
% ~\cite{DBLP:journals/pvldb/XingCCLOP24}
% hard code for this citation to keep the correct citation order
Empirical results demonstrate that our proposed technique reduces model selection time and computational expenses by up to 29.3$\times$ compared to existing model selection systems.
Moreover, we are actively developing \dbname, and the system implementation is still in progress. 
We shall report new experimental results as soon as they become available in the near future.
}


\vspace{-3mm}
\section{Response to Reviewer \#2}

% \begin{comment}
\comments{1}{
The current AI4DB actually is not fully deployed, partial due to the unstable results of AI techniques in handling the flexible input in DBMS. It is the Reliability metric in the paper. But I cannot see sufficient discussion to alleviate the issue.
}
% \end{comment}

\response{1}{
We agree that as data in the database evolves over time, static AI models can become inefficient in providing reliable results.
To alleviate this issue, as pointed out in Section~\ref{subsec:auto_overview}, we aim to design dynamic and online AI models that can be updated and adapted to data variations to maintain accuracy, thereby facilitating the continuous optimization of system components for better performance.
To achieve this, our core idea generally follows the FRP and employs online reinforcement learning (RL), which has been further discussed in Section~\ref{subsec:optimizer} and Section~\ref{subsec:cc}.
We have enhanced Section~\ref{subsec:auto_overview} to state this ideation more clearly.
% while minimizing the impact on system performance. 
% We therefore need to design new techniques to overcome these challenges.
% In particular, we aim to design dynamic and online AI models that facilitate continuous optimization of system components for better performance.
}


% \begin{comment}
\comments{2}{
It is better to provide the definition of Autonomous Data System at the beginning of the paper.
}
% \end{comment}

\response{2}{
Following your suggestion, we have defined the AI-powered Autonomous Data System in the Abstract and Section~\ref{sec:introduction} as a data system that provides in-database AI-powered analytics to seamlessly support AI applications, and fully embraces AI techniques in each major system component to offer self-driving capabilities.

% We have added a period to the index terms to address this issue in the revised paper.
}

% \begin{comment}
\comments{3}{
Figure 3 gives the conceptual framework of NeurDB, while NeurDB is in the left corner in the figure. The relationships between NeurDB to other components should be more clear.
}
% \end{comment}

\response{3}{
% Thank you for pointing out the issue.
As suggested, we have updated Figure~\ref{fig:overview} to indicate that \dbname includes Components \ding{172}\textasciitilde\ding{175}, which collaborate and interact with each other to effectively and efficiently support \ding{176} AI applications in various domains.
% These components correspond with and interact with each other to effectively and efficiently support AI-powered applications in various domains.
}


\vspace{-3mm}
\section{Response to Reviewer \#3}
% \begin{comment}
\comments{1}{
Figure 2 AI$\times$DB looks like the English character x. Using a mathematical cross would be better.
}

\response{1}{
Thank you for your careful review.
We have revised Figure~\ref{fig:history} as suggested.
% addressed this issue by adding a period to all the figure captions in the revised paper.
}


\comments{2}{
Sec 2.3.1 Intelligent healthcare: How does that relate to DB? Though e-commerce is built on DB, how does AI$\times$DB works in e-commerce? I don't see any explicit mention of DB problems in Sec 2.3.
}

\response{2}{
We have improved Section~\ref{sec:application} to clarify the relationship between modern AI applications and \dbname.
We envision that future intelligent healthcare and e-commerce applications can be efficiently managed by \dbname, eliminating the complexity of involving multiple dedicated systems for data management, model serving, etc.
Specifically, in the healthcare domain, the digital diagnosis system, where doctors and physicians record EMR data and other relevant patient and treatment information, can be constructed based on \dbname, which provides a mature infrastructure for fast data access and processing.
Since all the required data is stored in \dbname, applications such as AI-powered healthcare assistants can directly perform the necessary analysis within \dbname using its in-database AI-powered analytic capabilities.
Similarly, in the e-commerce sector, \dbname can be employed to support online purchases by maintaining tables such as the purchases data table with attributes (user, item, price).
Based on such data tables, we can conduct various predictive tasks, such as link prediction to indicate potential purchases and fraud detection, directly within \dbname.
}

\comments{3}{
In Figure 3, what's the relationship between different modules?
}

\response{3}{
\dbname includes Components \ding{172}\textasciitilde\ding{175}, which collaborate and interact with each other to effectively and efficiently support \ding{176} AI applications in various domains.
We have updated Figure~\ref{fig:overview} and the corresponding descriptions in Section~\ref{sec:framework} to state the relationship between different components more clearly.
}

\comments{4}{
Do you have reference for the claim at Page 3 Line 47: Databases have the potential to efficiently manage numerous AI models using their inherent user-friendly SQL interfaces, and provide high-quality data with their transaction guarantees to enhance AI model accuracy.
}

\response{4}{
To address your concern, we have added the corresponding citation for this sentence in Section~\ref{subsec:related_work}.
}

% \twocolumn

\clearpage

==> sections/abstract.tex <==



% Digitization and digitalization in multiple companies and organizations necessitate cross-institution data collaboration, aiming for improved profitability and sustainability.
% In facilitating such processes, a shared database system is typically employed for verifiable and efficient data sharing and collaboration.
% However, with insufficient consideration of the critical features pivotal to data collaboration, such as tamper evidence, data versioning, etc., existing solutions often come with suboptimal performance.

% In this paper, we 
% %present the design of 
% propose
% Distributed Fault-tolerant (DFT) Forkbase (\dbname)
% %\dbname provides tailored designs  to 
% which has been designed to
% support verifiable and efficient data collaboration under a practical threat model.
% Specifically,
% we propose a parallel execution algorithm to offer tamper evidence through high-performance \postree construction and traversal.
% In addition, \dbname employs a tree partitioning mechanism, ensuring efficient data versioning while minimizing storage overhead.
% %We enable 
% Further, it supports
% ACID transactions for the manipulation of various data types.
% %in \dbname.
% With the implementation of a fine-grained concurrency control algorithm, \dbname optimizes transaction throughput while effectively reducing abort rates.
% We conduct extensive experiments to compare {\dbname} against two baselines: OrpheusDB, a version management database, and Forkbase, a tamper-evident storage engine.
% The results show that \dbname achieves up to $4.5\times$ and $1.5\times$ higher throughput than OrpheusDB and Forkbase.


